Scalable Analysis of Urban Scaling Laws: Leveraging Cloud Computing to Analyze 21,280 Global Cities

Cities play a pivotal role in human development and sustainability, yet studying them presents significant challenges due to the vast scale and complexity of spatial-temporal data. One such challenge is the need to uncover universal urban patterns, such as the urban scaling law, across thousands of cities worldwide. In this study, we propose a novel large-scale geospatial data processing system that enables city analysis on an unprecedented scale. We demonstrate the system's capabilities by revisiting the urban scaling law across 21,280 cities globally, using a range of open-source datasets including road networks, nighttime light intensity, built-up areas, and population statistics. Analyzing the characteristics of 21,280 cities involves querying over half a billion geospatial data points, a task that traditional Geographic Information Systems (GIS) would take several days to process. In contrast, our cloud-based system accelerates the analysis, reducing processing time to just minutes while significantly lowering resource consumption. Our findings reveal that the urban scaling law varies across cities in under-developed, developing, and developed regions, extending the insights gained from previous studies focused on hundreds of cities. This underscores the critical importance of cloud-based big data processing for efficient, large-scale geospatial analysis. As the availability of satellite imagery and other global datasets continues to grow, the potential for scientific discovery expands exponentially. Our approach not only demonstrates how such large-scale tasks can be executed efficiently but also offers a powerful solution for data scientists and researchers working in the fields of city and geospatial science.

==> 6discovery-detail.tex <==

\subsection{Economic Development}

Accurate and comprehensive measurements of socioeconomic development are critical for research and policy.  Traditional approaches for measuring the key outcomes rely on infrequent and subjective (often biased) household surveys~\cite{burke2021using}. In recent years, many satellites have been launched to collect temporal, spatial, and spectral information on the Earth's surface. The abundance and high quality of satellite imagery stands in contrast to the inefficiency of survey data. Recently, there are rapidly growing scientific studies that seek to use satellite imagery to measure and understand outcomes
related to sustainable development. For example, an early study shows that nighttime light can be used as a proxy of economic statistics~\cite{chen2011using}. Later studies propose to use satellite imagery to help predict poverty~\cite{jean2016combining} and infer various sustainability measures such as economic status, agricultural and population~\cite{burke2021using}. However, none of these studies have targeted at global scale and examine the correlation between city properties and their economic status.

We calculate the correlation between city property and GDP.  We use the same GDP data~\cite{country-gdp} as in Section~\ref{sec:discovery:scale}. Since there is no GDP data at city level, we use the GDP of the country that the city belongs to. The cities in the same country will have the same GDP per capita.  


\begin{table}[htb]
    \centering
    \begin{tabular}{|c|c|c|}
        \hline
        City Property & Coefficient & $R^2$ \\ 
        \hline
        Road length & 0.589 & 0.266 \\
        Nighttime light & 1.012  & 0.534 \\
        Built-up surface area & 0.519 & 0.411 \\
        \hline
    \end{tabular}
    \caption{Correlation between city property per capita and GDP per capita for global cities. }
    \label{table:gdp_indicators}
\end{table}

The correlation between city property per capita and GDP per capita is shown in Table~\ref{table:gdp_indicators}. The correlation is calculated as a linear correlation after taking the natural logarithm on the two attributes. Overall, we see a positive correlation but the correlations are not strong.  This might due to coarse level of GDP data we are using. A finer scale of GDP data will be useful for a more in-depth analysis. 


\begin{table}[htb]
    \centering
    \begin{tabular}{|c|c|c|}
        \hline
        City & Country & Light per capita \\
        \hline
        Kalehe  & Congo & 6.16E-07\\
         Kabinda & Congo & 1.03E-06 \\
        Sabon Birni & Nigeria & 1.09E-06 \\
        Abim & Uganda & 1.65E-06 \\    
        Amuria &  Uganda & 1.79E-06\\      
        Silame & Nigeria & 1.93E-06\\
        Bukwo & Uganda & 2.21E-06 \\
        Binji &  Nigeria &  2.24E-06\\
        Tougué Prefecture & Guinea & 2.48E-06\\    
        Serere & Uganda & 2.51E-06 \\
        \hline
    \end{tabular}
    \caption{Top 10 cities with the lowest nighttime light per capita. }
    \label{table:lowest-light}
\end{table}

\begin{figure}[thb]
    \centering
    \includegraphics[width=0.45\textwidth]{figure/100cities-country.png}
    \caption{Number of cities in the top 100 cities with lowest nighttime light intensity for each country. The number above the bar indicates the count of cities per country.}
    \label{fig:100cities-country}
\end{figure}


Though the overall correlation is not strong, examination of individual cities reveals the relationships between city property and economic development.  Table~\ref{table:lowest-light} show 10 cities with the lowest nighttime light intensity per capita.
And if we examine 100 cities with lowest nighttime light intensities, they belong to only 15 countries. Figure~\ref{fig:100cities-country} shows the number of these cities for each country. From these results, we can see that the cities with very low nighttime light intensities all belong to underdeveloped countries.



